Spectral World Renderer: Unified 3D Hyperspectral Unmixing

Hyperspectral images (HSI) preserve material evidence lost in RGB, yet 3D material identification from multi-view HSI faces two obstacles. Spectral Gaussian splatting reconstructs spectra accurately but leaves unmixing to per-pixel post-processing, while multi-view hyperspectral capture is costly and real datasets lack pixel-level material labels and sub-pixel proportions. We propose Spectral World Renderer (SWR), a material-aware explicit representation that unifies 3D spectral reconstruction and unmixing: it fits a Gaussian scaffold from RGB and decodes ray-Gaussian intersections into abundances over a shared endmember dictionary. Additionally, appearance guidance prevents spectrally similar materials from merging when intensity absorbs their brightness differences. Moreover, SWR requires no material-label supervision during training. To address the data gap, we further construct the SWR Benchmark (SWR-Bench): a coding-agent pipeline generates eight indoor and outdoor worlds from measured reflectance, aligning HSI with both annotations. SWR achieves the highest mIoU in all eight worlds and the highest mean PSNR on each real dataset. On an 11-class urban world, it trains at least 3.67x faster than unmixing baselines; rendering averages 34.9 joint spectral and label views/s over four worlds on a single RTX 4090.

==> sec/3_1_swr_bench.tex <==
\par
% Fixed heading skips prevent flush-bottom stretching at this column break.
\makeatletter
\let\swrSavedSubsection\cvprsubsection
\def\cvprsubsection{\@startsection{subsection}{2}{\z@}{-6pt}{3pt}{\elvbf}}
\makeatother
\edef\swrSavedParskip{\the\parskip}
\setlength{\parskip}{1.5pt}
\subsection{World Generator and SWR-Bench}
\label{sec:swr}
\makeatletter
\let\cvprsubsection\swrSavedSubsection
\makeatother

SWR-Bench contains eight executable worlds, six outdoor and two indoor, from a palace and a market to a karst valley and an office (Figure~\ref{fig:data_pipeline}). They cover 5--11 material classes per world, 125 measured specimens and 1{,}404 views rendered at $960{\times}540$ with 64 bands. A coding agent (Claude Opus~5.5) writes each world as a scene program, and construction enforces three requirements: physical validity, verified by collision, support and clearance checks like SAGE~\citep{xia2026sage}; spectral realism, with reflectances matched to each material from public measured libraries~\citep{ecostress,kokaly2017usgs}; and sensor realism, with signal-dependent shot and read noise modelled on HSI sensors~\citep{foi2008noise,acito2011signal,meola2011modeling}, so training views reflect realistic acquisition.
\par\setlength{\parskip}{\swrSavedParskip}

\noindent\textbf{Reference-guided world generation.} We first give the coding agent a scene description and reference images that define the scene concept. To avoid arbitrary placement and reduce collisions, the agent then drafts a world map that fixes the layout~\citep{feng2023layoutgpt,yang2024holodeck} before writing the scene program with Model Context Protocol (MCP) tools~\citep{anthropic2024mcp} and agent skills; the renderer executes it with editable geometry, materials, lighting and cameras. Agents check rendered previews for structural support, object collisions and clearance and revise the program, completing generation and verification autonomously; a final human review then inspects each generated world.

\noindent\textbf{Shared-sample ground truth.} To avoid disagreements at silhouettes and mixed pixels, images and labels share the same $S$ sub-pixel camera samples ($S=16$): for the pixel indexed by ray $\mathbf r$, $\mathbf x_n$ is the first surface hit of sample $n$ and $\mathcal M(\mathbf x_n)$ its material class. A Lambertian specimen $j$ with measured reflectance $\rho_j(\lambda)$ at wavelength $\lambda$ has, under direct or sky illumination $u$, band radiance
\begin{equation}
 v^u_{j,\ell}=\int \psi_\ell(\lambda)\,\rho_j(\lambda)\Phi_u(\lambda)/\pi\,\mathrm d\lambda,\quad u\in\{\mathrm d,\mathrm s\},
 \label{eq:formation}
\end{equation}
where $\psi_\ell$ is the response of band $\ell$ and $\Phi_{\mathrm d},\Phi_{\mathrm s}$ are direct and sky irradiance. The vectors $\mathbf v_j^u\in\mathbb R^L$ and shading coefficients $C_j^u(\mathbf r)$, averaged over the $S$ samples, give
\begin{equation}
 \begin{aligned}
 \mathbf H_{\mathrm{clean}}(\mathbf r)&=\textstyle\sum_j(C_j^{\mathrm d}(\mathbf r)\mathbf v_j^{\mathrm d}+C_j^{\mathrm s}(\mathbf r)\mathbf v_j^{\mathrm s}),\\
 A_c(\mathbf r)&=\tfrac1S\textstyle\sum_{n=1}^{S}[\mathcal M(\mathbf x_n)=c].
 \end{aligned}
 \label{eq:gt}
\end{equation}
Here $[\cdot]$ is the indicator function, $c$ indexes $C$ material classes and $j$ measured specimens. Area proportions renormalize $A_c$ over non-sky samples. Learned endmembers use index $k$ and need not correspond one-to-one to classes. Some worlds extend this model with specular reflection, water or path-traced indoor light transport in Mitsuba~\citep{mitsuba3}.

\looseness=-1
\noindent\textbf{Measured spectra and variability.} ECOSTRESS and USGS specimens give each material a traceable measured spectrum; several specimens per class add within-class variability, fixed per surface across views (Figure~\ref{fig:swr_spectra}(a,b)). Illumination uses ASTM G173 sunlight and skylight~\citep{astmg173} and CIE white sources~\citep{cie2018colorimetry}, giving standard irradiance for natural and artificial light. Clean and noisy 64-band cubes (420--980\,nm) serve evaluation and training.

\noindent\textbf{Verification.} Finally, we verify label alignment, spectral provenance and split separation. Specifically, the per-term contributions re-compose clean outdoor radiance, while indoor transport is checked before noise. Figure~\ref{fig:swr_spectra}(c) compares assigned spectra with independent library measurements.

